Improving Document Representations by Generating Pseudo Query Embeddings for Dense Retrieval

Recently, the retrieval models based on dense representations have been gradually applied in the first stage of the document retrieval tasks, showing better performance than traditional sparse vector space models. To obtain high efficiency, the basic structure of these models is Bi-encoder in most cases. However, this simple structure may cause serious information loss during the encoding of documents since the queries are agnostic. To address this problem, we design a method to mimic the queries on each of the documents by an iterative clustering process and represent the documents by multiple pseudo queries (i.e., the cluster centroids). To boost the retrieval process using approximate nearest neighbor search library, we also optimize the matching function with a two-step score calculation procedure. Experimental results on several popular ranking and QA datasets show that our model can achieve state-of-the-art results.

==> equation.tex <==
Although the performance of the ranking metrics like MRR can show the effectiveness of the our method. We still lack an in-depth view of why our cluster centroid based embeddings are better than other document embeddings (e.g., the first-m token embeddings or randomly selected token embeddings). In this section, we try to find the reason by analyzing how the document embeddings affect the value of the loss function.

Given a query $q$ and one of its relative document $d$, the training objective is to minimize the loss function in the following form:
\begin{equation}
    \mathcal{L} = -{\log{\text{softmax}(y_d)}} 
\end{equation}
where $y_d$ is computed as Eq. \ref{eq:6}. Next, we can see how a single step of gradient descent alters the loss value by analyzing the gradient of the loss function with respect to the document embeddings. For each document embedding $c_j$, we have:
\begin{align}
    \triangledown_d \mathcal{L}_d = & (y_d-1)e_q\triangledown e_d \\
    \triangledown_j e_d = & r(c_j)\triangledown c_j \\
    r(c_j) = & [1 + (\sum_{j'\neq j}a_{j'}(e_q c_j - e_q c_{j'}))]a_j
\end{align}
where $\triangledown_d \mathcal{L}$ means the gradient of loss with respect to document $d$ and $\triangledown_j e_d$ means the gradient of $e_d$ with respect to $c_j$. Details of the derivation are shown in the Appendix. Intuitively, if $r(c_j)$ is positive, moving $c_j$ towards the direction defined by $\triangledown c_j$ has a positive impact on reducing the loss, and if $r(c_j)$ is negative, it will has a negative impact on reducing the loss. The absolute value of $r(c_j)$ can be interpreted as a weight of how much the $c_j$ can contribute to the loss value. For example, if we feed the model with document embedding producing large positive $r(c_j)$, a single gradient descent step would decrease the loss value faster than small $r(c_j)$. 

% From Eq. 16 we can see that $r(c_j)$ would be relatively high if the document embedding $c_j$ approximates to $e_q$ (higher $e_q c_j$ and $a_j$) and other document embeddings $c_{j'\neq j}$ are far from $e_q$ (lower $e_q c_{j'}$ and $a_{j'}$). 

To verify whether the cluster centroids are more effective than other document embeddings, we compare our model with two other models: the first one adopts the first-$k$ token embeddings as the document embeddings like Poly-Encoder(first-$k$)\cite{poly2019} and the second one adopts $k$ randomly selected token embeddings as the document embeddings. Other parts of the model remain unchanged. Ideally, we expect (1) at least one of the document embeddings can match its relative query embedding and (2) multiple document embeddings can capture different semantic information of the document. We use the max value of $r(c_j)$ among multiple document embeddings to evaluate (1) and use the variance of $r(c_j)$ among the multiple embeddings of the same document to evaluate (2). We plot them during the training as shown in Figure \ref{fig:values of model}.

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{acl-ijcnlp2021-templates/pics/loss.png}
         \caption{Loss function value.}
         \label{fig:loss}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{acl-ijcnlp2021-templates/pics/maxcj.png}
         \caption{$\text{max}(r(c_j))$.}
         \label{fig:maxcj}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{acl-ijcnlp2021-templates/pics/varcj.png}
         \caption{$\text{var}(r(c_j))$.}
         \label{fig:varcj}
     \end{subfigure}
        \caption{Loss, $\text{max}(r(c_j))$ and $\text{var}(r(c_j))$ of different models.}
        \label{fig:values of model}
\end{figure*}

At the beginning of the training, both $\text{max}(r(c_j))$ and $\text{var}(r(c_j))$ are relatively high and sharply decrease with the loss value. Since the training is at a preliminary stage, it is easy to find a direction to reduce the loss value. When the decreasing of the loss slows down, our model can provide a much higher $\text{max}(r(c_j))$ which dominates the loss to decrease more than other two models. Besides, $\text{var}(r(c_j))$ of our model is also higher than others indicating the document embeddings are different with each other. Overall, we conclude that our model produces diverse document embeddings which make it easier to reduce the loss thus achieving a better model. 

















